Contrastive Learning of Temporal Distinctiveness for Survival Analysis in Electronic Health Records

Survival analysis plays a crucial role in many healthcare decisions, where the risk prediction for the events of interest can support an informative outlook for a patient's medical journey. Given the existence of data censoring, an effective way of survival analysis is to enforce the pairwise temporal concordance between censored and observed data, aiming to utilize the time interval before censoring as partially observed time-to-event labels for supervised learning. Although existing studies mostly employed ranking methods to pursue an ordering objective, contrastive methods which learn a discriminative embedding by having data contrast against each other, have not been explored thoroughly for survival analysis. Therefore, in this paper, we propose a novel Ontology-aware Temporality-based Contrastive Survival (OTCSurv) analysis framework that utilizes survival durations from both censored and observed data to define temporal distinctiveness and construct negative sample pairs with adjustable hardness for contrastive learning. Specifically, we first use an ontological encoder and a sequential self-attention encoder to represent the longitudinal EHR data with rich contexts. Second, we design a temporal contrastive loss to capture varying survival durations in a supervised setting through a hardness-aware negative sampling mechanism. Last, we incorporate the contrastive task into the time-to-event predictive task with multiple loss components. We conduct extensive experiments using a large EHR dataset to forecast the risk of hospitalized patients who are in danger of developing acute kidney injury (AKI), a critical and urgent medical condition. The effectiveness and explainability of the proposed model are validated through comprehensive quantitative and qualitative studies.

==> tex/graphics.tex <==




\begin{figure}[t]
\begin{center}
%\centering
%\vspace{-3ex}
%\includegraphics[width=0.5\linewidth]{figures/simple-system.pdf}
\includegraphics[width=1.0\linewidth]{tex/km_baselines2.pdf}
\caption{Mean survival curve comparison}
\label{fig:km-baselines}
%\vspace{-4ex}
\end{center}
\end{figure}


\begin{figure}[t]
\begin{center}
%\centering
%\vspace{-3ex}
%\includegraphics[width=0.5\linewidth]{figures/simple-system.pdf}
\includegraphics[width=1.0\linewidth]{tex/km_baselines_interpolate2.pdf}
\caption{Mean survival curve comparison (interpolated)}
\label{fig:km-baseline_interpolated}
%\vspace{-4ex}
\end{center}
\end{figure}



\begin{figure}[t]
\begin{center}
%\centering
%\vspace{-3ex}
%\includegraphics[width=0.5\linewidth]{figures/simple-system.pdf}
\includegraphics[width=1.0\linewidth]{tex/km_baselines_ob2.pdf}
\caption{Mean survival curve comparison only for observed patients}
\label{fig:km-baselines-ob}
%\vspace{-4ex}
\end{center}
\end{figure}


\begin{figure}[t]
\begin{center}
%\centering
%\vspace{-3ex}
%\includegraphics[width=0.5\linewidth]{figures/simple-system.pdf}
\includegraphics[width=1.0\linewidth]{tex/km_baselines_ob_interpolate2.pdf}
\caption{Mean survival curve comparison only for observed patients (interpolated)}
\label{fig:km-baselines-ob-interpolated}
%\vspace{-4ex}
\end{center}
\end{figure}


\begin{figure}[t]
\begin{center}
%\centering
%\vspace{-3ex}
%\includegraphics[width=0.5\linewidth]{figures/simple-system.pdf}
\includegraphics[width=1.0\linewidth]{km-ob2.pdf}
\caption{Estimated survival curve for an observed patient}
\label{fig:km-ob2}
%\vspace{-4ex}
\end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
%\centering
%\vspace{-3ex}
%\includegraphics[width=0.5\linewidth]{figures/simple-system.pdf}
\includegraphics[width=1.0\linewidth]{tex/drug_attention.pdf}
\caption{Attention weights of drug codes inside the last visit of an observed patient}
\label{fig:drug_attention}
%\vspace{-4ex}
\end{center}
\end{figure}


\begin{figure}[t]
\begin{center}
%\centering
%\vspace{-3ex}
%\includegraphics[width=0.5\linewidth]{figures/simple-system.pdf}
\includegraphics[width=1.0\linewidth]{tex/diag_attention.pdf}
\caption{Attention weights of visits and attention weights of diagnosis codes inside each visit.}
\label{fig:diag_attention}
%\vspace{-4ex}
\end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
%\centering
%\vspace{-3ex}
%\includegraphics[width=0.5\linewidth]{figures/simple-system.pdf}
\includegraphics[width=1.0\linewidth]{mean_surv_interpolate_ob2_2.pdf}
\caption{Attention weights of visits and attention weights of diagnosis codes inside each visit.}
\label{fig:mean-surv}
%\vspace{-4ex}
\end{center}
\end{figure}


